On the Duality of Semiantichains and Unichain Coverings

We study a min-max relation conjectured by Saks and West: For any two posets $P$ and $Q$ the size of a maximum semiantichain and the size of a minimum unichain covering in the product $P\times Q$ are equal. For positive we state conditions on $P$ and $Q$ that imply the min-max relation. Based on these conditions we identify some new families of posets where the conjecture holds and get easy proofs for several instances where the conjecture had been verified before. However, we also have examples showing that in general the min-max relation is false, i.e., we disprove the Saks-West conjecture.

==> pic-bad_example.tex <==
% rysunek prezentujacy kontrprzyklad

\tikzstyle vertex=[circle, line width=0.15mm, draw, fill=black, inner sep=0pt, minimum width=2.2mm]%

%\draw (0,0) rectangle (10,4.5) ;
%\draw (0,0) node (1d) {};
\foreach \x in {0,...,4} {
	\draw (\x,0) node[vertex] (d\x) [label=left:$\the\numexpr\x+6\relax$] {};
	\draw (\x-1,1) node[vertex] (u\x) [label=above:$\the\numexpr\x+1\relax$] {};
}

\foreach \x in {1,2,3} {
	\draw (\x,-1) node[vertex] (s\x) [label=below:$\the\numexpr\x+10\relax$] {};
}

\foreach \x in {0,...,4} {
	\foreach \y in {1,2,3} {
		\draw (d\x) -- (s\y);
	}
}

\draw (u0) -- (d0);
\draw (u1) -- (d0);
\draw (u2) -- (d0);
\draw (u2) -- (d1);
\draw (u2) -- (d2);
\draw (u3) -- (d2);
\draw (u4) -- (d2);
\draw (u4) -- (d3);
\draw (u4) -- (d4);


\draw (5.5,0) node[vertex] (v1) [label=above:$b$] {};
\draw (6.5,0) node[vertex] (v2) [label=above:$c$] {};
\draw (6,-1) node[vertex] (v0) [label=below:$a$] {};

\draw (v1) -- (v0) -- (v2);

\draw  (-.5,-.5) node {$P$};
\draw  (5,-.5) node {$Q$};


==> updfig <==
#! /bin/csh -f

# cd Figures

fig2dev -L pdftex $1.fig > $1.pdf
fig2dev -L pstex $1.fig > $1.eps

fig2dev -L pstex_t -p $1.pstex $1.fig > $1.pstex_t

perl -p -i.bak -e 's#.pstex##g' $1.pstex_t

perl -p -i.bak -e 's#\\begingroup#\n\\multiply\\unitlength by \\magproz\n\\divide\\unitlength by 100\n\n\\begingroup#g' $1.pstex_t

perl -p -i.bak -e 's#\includegraphics{#\includegraphics[scale=\\figscale]{#g' $1.pstex_t

rm $1.pstex_t.bak

# cd ..

##############################
# new version of UPDPSF 
# renamed to UPDFIG
# new feature, generates pdf and eps and doesn't specify
# which to include. So everything can be used with
# latex and pdflatex without any change.

